Spatially resolved random telegraph fluctuations of a single trap at the Si/SiO2 interface

We use electrostatic force microscopy to spatially resolve random telegraph noise at the Si/SiO$_2$ interface. Our measurements demonstrate that two-state fluctuations are localized at interfacial traps, with bias-dependent rates and amplitudes. These two-level systems lead to correlated carrier number and mobility fluctuations with a range of characteristic timescales; taken together as an ensemble, they give rise to a $1/f$ power spectral trend. Such individual defect fluctuations at the Si/SiO$_2$ interface impair the performance and reliability of nanoscale semiconductor devices, and will be a significant source of noise in semiconductor-based quantum sensors and computers. The fluctuations measured here are associated with a four-fold competition of rates, including slow two-state switching on the order of seconds and, in one state, fast switching on the order of nanoseconds which is associated with energy loss.

==> _Notes.tex <==
\subsection*{Manuscript Length}

A standard 6-page article is approximately 4,000 words, 50 references, and 4 medium-size graphical elements (i.e., figures and tables). The preferred length of articles remains at 6 pages, but PNAS will allow articles up to a maximum of 12 pages.


\subsection*{Data Archival}

PNAS must be able to archive the data essential to a published article. Where such archiving is not possible, deposition of data in public databases, such as GenBank, ArrayExpress, Protein Data Bank, Unidata, and others outlined in the \href{https://www.pnas.org/author-center/editorial-and-journal-policies#materials-and-data-availability}{Information for Authors}, is acceptable.


\subsection*{Supporting Information Appendix (SI)}

Authors should submit SI as a single separate SI Appendix PDF file, combining all text, figures, tables, movie legends, and SI references. SI will be published as provided by the authors; it will not be edited or composed. Additional details can be found in the \href{https://www.pnas.org/authors/submitting-your-manuscript#manuscript-formatting-guidelines}{PNAS Author Center}. The PNAS Overleaf SI template can be found \href{https://www.overleaf.com/latex/templates/pnas-template-for-supplementary-information/wqfsfqwyjtsd}{here}. Refer to the SI Appendix in the manuscript at an appropriate point in the text. Number supporting figures and tables starting with S1, S2, etc.


\subsubsection*{SI Datasets}

Supply .xlsx, .csv, .txt, .rtf, or .pdf files. This file type will be published in raw format and will not be edited or composed.


\subsubsection*{SI Movies}

Supply Audio Video Interleave (avi), Quicktime (mov), Windows Media (wmv), animated GIF (gif), or MPEG files. Movie legends should be included in the SI Appendix file. All movies should be submitted at the desired reproduction size and length. Movies should be no more than 10MB in size.

